Growing Pains: Understanding the Impact of Likelihood Uncertainty on Hierarchical Bayesian Inference for Gravitational-Wave Astronomy

Observations of gravitational waves emitted by merging compact binaries have provided tantalising hints about stellar astrophysics, cosmology, and fundamental physics. However, the physical parameters describing the systems, (mass, spin, distance) used to extract these inferences about the Universe are subject to large uncertainties. The most widely-used method of performing these analyses requires performing many Monte Carlo integrals to marginalise over the uncertainty in the properties of the individual binaries and the survey selection bias. These Monte Carlo integrals are subject to fundamental statistical uncertainties. Previous treatments of this statistical uncertainty has focused on ensuring the precision of the inferred inference is unaffected, however, these works have neglected the question of whether sufficient accuracy can also be achieved. In this work, we provide a practical exploration of the impact of uncertainty in our analyses and provide a suggested framework for verifying that astrophysical inferences made with the gravitational-wave transient catalogue are accurate. Applying our framework to models used by the LIGO-Virgo-KAGRA collaboration and in the wider literature, we find that Monte Carlo uncertainty in estimating the survey selection bias is the limiting factor in our ability to probe narrow population models and this will rapidly grow more problematic as the size of the observed population increases.

==> solutions.tex <==
\section{\label{sec:combining-catalogs}Combining catalogs}

Since the variance in the likelihood scales linearly with the size of the considered population it is tempting to ask ``can we just analyze smaller sub-populations with a small number of samples per event and then combine these measurements?''
The answer is a resounding ``maybe''.
This approach hinges on having a viable method to combine multiple results obtained from distinct catalogs.
In order to do this it is necessary to assume that all of the population parameters ($\Lambda$) have the same shared values across all subcatalogs, i.e., we introduce an additional layer into our hierarchy where the top-level model is a delta function.
This requires some care in the choice of method to split the full dataset to avoid subtle biases.
For gravitational-wave transient populations, we suggest splitting based on the arrival time of the signals, e.g., analyze all events from each month individually and then combine.
We can then write our full likelihood
\begin{equation}
    p(\{\{d\}_i\} | \Lambda) = \prod^{N_{\rm chunks}}_{i} p(\{d\}_i | \Lambda).
\end{equation}
Where $N_{\rm chunks}$ is the number of sub-catalogs.

The first approach someone familiar with population inference for gravitational-wave transients may take is to simply take the posterior samples for each sub-catalog and importance sample them based on the likelihood for the other catalogs.
This method is unsatisfactory as there is no new added information and so the uncertainty in the final likelihoods will still maintain the original uncertainties and hence require the same, large, number of samples per event in order to be combined.

We propose a different approach to combining catalogs relying on an assumption that the posterior distribution for the population parameters is smooth (or can be made smooth through an appropriate transformation.)
With this assumption, we can combine smooth fits to the sub-catalog likelihoods and the uncertainty in the global fit will be compressed like $\sqrt{N_{\rm chunks}}$.

We note that this approach is similar in spirit to previously considered methods~\cite{Biscoveanu2020, Isi2019} to approximate the delta function population model population model from discrete samples.
Since a delta function cannot be used as the target distribution for importance sampling, these approaches specify a Gaussian kernel and identify the limit $\sigma \rightarrow 0 $ as the desired result.
While this is useful as a consistency test between sub-catalogs, importance sampling to a narrow population model is difficult as demonstrated in previous sections.

\section{\label{sec:joint-fitting}Simultaneous sampling for individual event and population parameters}

As an alternative to performing Monte Carlo integrals over the single event parameters, we can instead marginalize over these parameters using MCMC methods.
This involves simultaneously sampling over the population hyperparameters and the single event parameters.
The total dimensionality of this space will be $d = M_{\Lambda} + N_{\rm events} M_{\theta}$.
For a naive MCMC implementation, the scaling with dimensionality is ${\cal O}(d^2) \sim {\cal O}(N^2_{\rm events})$.
Hamiltonian Monte Carlo can perform better, reaching approximately ${\cal O}(d^{5/4}) \sim {\cal O}(N^{5/4}_{\rm events})$, however, this method requires the target density to be differentiable (either analytically or numerically).
We note that the likelihood can be efficiently divided into (approximately) independent blocks.
For fixed hyperparameters, the likelihood exactly factors between events.
By employing blocked Gibbs sampling, we can reduce the scaling to ${\cal O}(M^2_{\Lambda} + N_{\rm events} M^2_{\theta}) \sim {\cal O}(N_{\rm events})$.

Another, implementation issue with sampling the full $d$ dimensional space is the necessity to evaluate the single-event likelihoods at each step.
Typically, this involves generating a model waveform and comparing to observed strain.
By approximating the single-event likelihood marginalized over nuisance parameters, we can compute this likelihood without an expensive waveform evaluation.

